Azimuthal asymmetry in the risetime of the surface detector signals of the Pierre Auger Observatory

The azimuthal asymmetry in the risetime of signals in Auger surface detector stations is a source of information on shower development. The azimuthal asymmetry is due to a combination of the longitudinal evolution of the shower and geometrical effects related to the angles of incidence of the particles into the detectors. The magnitude of the effect depends upon the zenith angle and state of development of the shower and thus provides a novel observable, $(\sec \theta)_\mathrm{max}$, sensitive to the mass composition of cosmic rays above $3 \times 10^{18}$ eV. By comparing measurements with predictions from shower simulations, we find for both of our adopted models of hadronic physics (QGSJETII-04 and EPOS-LHC) an indication that the mean cosmic-ray mass increases slowly with energy, as has been inferred from other studies. However, the mass estimates are dependent on the shower model and on the range of distance from the shower core selected. Thus the method has uncovered further deficiencies in our understanding of shower modelling that must be resolved before the mass composition can be inferred from $(\sec \theta)_\mathrm{max}$.

==> 2016-01-author_list_latex_institutions.tex <==
% created on 2016-01-11

\begin{description}[labelsep=0.2em,align=right,labelwidth=0.7em,labelindent=0em,leftmargin=2em,noitemsep]
\item[$^{1}$] Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), Argentina
\item[$^{2}$] Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Argentina
\item[$^{3}$] Departamento de F\'\i{}sica, FCEyN, Universidad de Buenos Aires, Argentina
\item[$^{4}$] IFLP, Universidad Nacional de La Plata and CONICET, Argentina
\item[$^{5}$] Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Argentina
\item[$^{6}$] Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Argentina
\item[$^{7}$] Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM) and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Argentina
\item[$^{8}$] Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Centro At\'omico Constituyentes, Comisi\'on Nacional de Energ\'\i{}a At\'omica, Argentina
\item[$^{9}$] Observatorio Pierre Auger, Argentina
\item[$^{10}$] Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Argentina
\item[$^{11}$] Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Argentina
\item[$^{12}$] University of Adelaide, Australia
\item[$^{13}$] Centro Brasileiro de Pesquisas Fisicas (CBPF), Brazil
\item[$^{14}$] Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Brazil
\item[$^{15}$] Universidade de S\~ao Paulo, Inst.\ de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, Brazil
\item[$^{16}$] Universidade de S\~ao Paulo, Inst.\ de F\'\i{}sica, S\~ao Paulo, Brazil
\item[$^{17}$] Universidade Estadual de Campinas (UNICAMP), Brazil
\item[$^{18}$] Universidade Estadual de Feira de Santana (UEFS), Brazil
\item[$^{19}$] Universidade Federal da Bahia, Brazil
\item[$^{20}$] Universidade Federal de Pelotas, Brazil
\item[$^{21}$] Universidade Federal do ABC (UFABC), Brazil
\item[$^{22}$] Universidade Federal do Paran\'a, Setor Palotina, Brazil
\item[$^{23}$] Universidade Federal do Rio de Janeiro (UFRJ), Instituto de F\'\i{}sica, Brazil
\item[$^{24}$] Universidade Federal Fluminense, Brazil
\item[$^{25}$] Universidad Industrial de Santander, Colombia
\item[$^{26}$] Institute of Physics (FZU) of the Academy of Sciences of the Czech Republic, Czech Republic
\item[$^{27}$] Palacky University, RCPTM, Czech Republic
\item[$^{28}$] University Prague, Institute of Particle and Nuclear Physics, Czech Republic
\item[$^{29}$] Institut de Physique Nucl\'eaire d'Orsay (IPNO), Universit\'e Paris 11, CNRS-IN2P3, France
\item[$^{30}$] Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, France
\item[$^{31}$] Laboratoire de Physique Subatomique et de Cosmologie (LPSC), Universit\'e Grenoble-Alpes, CNRS/IN2P3, France
\item[$^{32}$] Station de Radioastronomie de Nan\c{c}ay, France
\item[$^{33}$] SUBATECH, \'Ecole des Mines de Nantes, CNRS-IN2P3, Universit\'e de Nantes, France
\item[$^{34}$] Bergische Universit\"at Wuppertal, Fachbereich C -- Physik, Germany
\item[$^{35}$] Karlsruhe Institute of Technology, Institut f\"ur Experimentelle Kernphysik (IEKP), Germany
\item[$^{36}$] Karlsruhe Institute of Technology, Institut f\"ur Kernphysik (IKP), Germany
\item[$^{37}$] Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik (IPE), Germany
\item[$^{38}$] RWTH Aachen University, III.\ Physikalisches Institut A, Germany
\item[$^{39}$] Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Germany
\item[$^{40}$] Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Germany
\item[$^{41}$] INAF -- Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy
\item[$^{42}$] INFN Laboratori del Gran Sasso, Italy
\item[$^{43}$] INFN, Sezione di Catania, Italy
\item[$^{44}$] INFN, Sezione di L'Aquila, Italy
\item[$^{45}$] INFN, Sezione di Lecce, Italy
\item[$^{46}$] INFN, Sezione di Milano, Italy
\item[$^{47}$] INFN, Sezione di Napoli, Italy
\item[$^{48}$] INFN, Sezione di Roma "Tor Vergata", Italy
\item[$^{49}$] INFN, Sezione di Torino, Italy
\item[$^{50}$] Osservatorio Astrofisico di Torino (INAF), Torino, Italy
\item[$^{51}$] Universit\`a Torino, Dipartimento di Fisica, Italy
\item[$^{52}$] Universit\`a del Salento, Dipartimento di Ingegneria, Italy
\item[$^{53}$] Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Italy
\item[$^{54}$] Universit\`a dell'Aquila, Dipartimento di Chimica e Fisica, Italy
\item[$^{55}$] Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Italy
\item[$^{56}$] Universit\`a di Milano, Dipartimento di Fisica, Italy
\item[$^{57}$] Universit\`a di Napoli "Federico II", Dipartimento di Fisica, Italy
\item[$^{58}$] Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Italy
\item[$^{59}$] Benem\'erita Universidad Aut\'onoma de Puebla (BUAP), M\'exico
\item[$^{60}$] Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico
\item[$^{61}$] Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico
\item[$^{62}$] Universidad Aut\'onoma de Chiapas, M\'exico
\item[$^{63}$] Universidad Michoacana de San Nicol\'as de Hidalgo, M\'exico
\item[$^{64}$] Universidad Nacional Aut\'onoma de M\'exico, M\'exico
\item[$^{65}$] Institute for Mathematics, Astrophysics and Particle Physics (IMAPP), Radboud Universiteit, Nijmegen, Netherlands
\item[$^{66}$] KVI -- Center for Advanced Radiation Technology, University of Groningen, Netherlands
\item[$^{67}$] Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Netherlands
\item[$^{68}$] Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, Netherlands
\item[$^{69}$] Institute of Nuclear Physics PAN, Poland
\item[$^{70}$] University of \L{}\'od\'z, Poland
\item[$^{71}$] Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Portugal
\item[$^{72}$] ``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Romania
\item[$^{73}$] Institute of Space Science, Romania
\item[$^{74}$] University of Bucharest, Physics Department, Romania
\item[$^{75}$] University Politehnica of Bucharest, Romania
\item[$^{76}$] Experimental Particle Physics Department, J.\ Stefan Institute, Slovenia
\item[$^{77}$] Laboratory for Astroparticle Physics, University of Nova Gorica, Slovenia
\item[$^{78}$] Universidad Complutense de Madrid, Spain
\item[$^{79}$] Universidad de Granada and C.A.F.P.E., Spain
\item[$^{80}$] Universidad de Santiago de Compostela, Spain
\item[$^{81}$] Case Western Reserve University, USA
\item[$^{82}$] Colorado School of Mines, USA
\item[$^{83}$] Colorado State University, USA
\item[$^{84}$] Department of Physics and Astronomy, Lehman College, City University of New York, USA
\item[$^{85}$] Fermi National Accelerator Laboratory, USA
\item[$^{86}$] Louisiana State University, USA
\item[$^{87}$] Michigan Technological University, USA
\item[$^{88}$] New York University, USA
\item[$^{89}$] Northeastern University, USA
\item[$^{90}$] Ohio State University, USA
\item[$^{91}$] Pennsylvania State University, USA
\item[$^{92}$] University of Chicago, USA
\item[$^{93}$] University of Hawaii, USA
\item[$^{94}$] University of Nebraska, USA
\item[$^{95}$] University of New Mexico, USA
\item[$^{a}$] School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom
\item[$^{b}$] Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany
\item[$^{c}$] also at Vrije Universiteit Brussels, Brussels, Belgium
\item[$^{d}$] also at Deutsches Elektronen-Synchrotron (DESY), Zeuthen, Germany
\end{description}

